Label Mapping Neural Networks with Response Consolidation for Class Incremental Learning

Class incremental learning refers to a special multi-class classification task, in which the number of classes is not fixed but is increasing with the continual arrival of new data. Existing researches mainly focused on solving catastrophic forgetting problem in class incremental learning. To this end, however, these models still require the old classes cached in the auxiliary data structure or models, which is inefficient in space or time. In this paper, it is the first time to discuss the difficulty without support of old classes in class incremental learning, which is called as softmax suppression problem. To address these challenges, we develop a new model named Label Mapping with Response Consolidation (LMRC), which need not access the old classes anymore. We propose the Label Mapping algorithm combined with the multi-head neural network for mitigating the softmax suppression problem, and propose the Response Consolidation method to overcome the catastrophic forgetting problem. Experimental results on the benchmark datasets show that our proposed method achieves much better performance compared to the related methods in different scenarios.

==> 002_related_work.tex <==
\section{Related Work}
\label{related_work}

There have been many studies focusing on class incremental problem and other related fields.  In this section, we will analyze the contributions and limitations of these methods in detail.

\subsection{Class Incremental Learning}
Most of existing class incremental learning models are based on the Rehearsal as introduced in Sec.~\ref{introduction}.
 According to the method used to access the data of the old classes, these approaches can be divided into two categories.

The first is data pool.
This kind of approaches needs to store a part of previous data containing old classes. 
Robins, et al.\cite{robins1998catastrophic} proposed Rehearsal and pseudo-rehearsal methods, which replay the old data to retrain the model. 
% However, it is evident that storing the original training samples is not efficient.
% Therefore, there are also other ways to store the compressed information of old data rather than original training samples.
Rebuffi, et al.\cite{rebuffi2017icarl:} leverages the deep learning model and Nearest-Mean-of-Exemplars method to classify the incremental classes in data pool.   
Castro, et al.\cite{castro2018end-to-end} proposed an End-to-End class incremental learning network using LwF and the auxiliary of data pool.
Mu, et al.\cite{mu2017streaming} proposed using low-dimensional matrix sketches as the summarization of existing classes data.
Anyway, these methods always require a amount of storage space to cache a part of data of the old classes. 
% In addition, compressing the data of the old classes on some complicated datasets, such as ImageNet, is also difficult.

% Similarly,  SOM \cite{kohonen1989self-organized} and SOINN \cite{shen2008a} can also generate prototype samples incrementally to cope with class incremental task.

The other family of methods utilizes the generative models to generate pseudo samples of the old classes.
Deep Generative Replay (DGR) \cite{shin2017continual} trains a Generative Adversary Network (GAN) \cite{goodfellow2014generative} model to help training the classification model.
GAN is also used in \cite{wu2018incremental} to generate auxiliary training data.
Ven,  et al.~\cite{van2018generative} modified the DGR by leveraging the Variational AutoEncoder (VAE) \cite{kingma2014auto-encoding} and distilling \cite{hinton2015distilling}.
These methods can greatly improve the space efficiency because they need not cache the old classes. 
However, before training classification model, we must wait for the generative model to generate a large amount of pseudo data of old classes,  which is inefficient in time. 
In addition, the load of  training classification model is not alleviated because the old classes are still included in the training set.
% In addition, such methods heavily rely on the performance of generative models.

\subsection{Catastrophic Forgetting Problem}

Catastrophic forgetting is a long-standing problem. 
This problem does not only occur in class incremental task, but also in other fields such as task incremental learning and reinforcement continual learning.
To deal with this problem, Goodfellow, et al.~\cite{goodfellow2014an} made an empirical study on the different activation functions and dropout layer for preventing the catastrophic forgetting.
EWC \cite{kirkpatrick2017overcoming} consolidates the important weights measured by Fisher information matrix.
\cite{zenke2017continual} proposed Synaptic Intelligence (SI), which accumulates and exploits task relevant information over time to prevent forgetting.
 LwF~\cite{li2017learning} was proposed by means of distilling on task incremental learning.
Rusu, et al.~\cite{rusu2017progressive} proposed progressive network which stacks previous neural networks to keep the memory of old data.
\cite{fernando2017pathnet} further proposed the Pathnet using tournament selection genetic algorithm.
\cite{xiao2014error-driven} proposed an Error-driven method which grows a network not only incrementally but also hierarchically.

% \subsection{Task incremental Learning }
% Task incremental deep learning aims to train a Multi-task neural network, but the tasks are given in sequential style.   Multi-task model leverages useful information contained in multiple related tasks to help improve the generalization of all tasks \cite{zhang2017a}. Multi-task deep learning model is typically composed of  a multi-head neural network. Each head is \textbf{independently} responsible for a single task. More details can be referred in \cite{ruder2017overview}.

% In \cite{van2018generative}, the authors clearly distinguished the difference between task incremental learning and class incremental learning.  In fact, class incremental learning is more difficult because of the softmax suppression problem.  Multi-task deep learning model has multiple heads,  Nevertheless, in class incremental learning, new categories is joint with the old categories which cannot be distinguished. This is why softmax suppression exists because the new categories and old categories are no independent when training.






==> 005_discussion.tex <==
\section{Discussion}
\subsection{Class Incremental Setup}
Non-overlapping sets of classes are typical experimental setup in almost related work of class incremental learning\cite{}. Therefore we also followed this conventional testing protocol in our experiments.
 It is worth note that this experimental setup represents the hardest situation, where the catastrophic forgetting phenomenon is the most obvious. 
However, in the real-world scenario, the new classes and the old classes are always mixed up together in the data streaming.
Under the circumstances, we can decompose this scenario into two parts. The first one is training the new classes on the new head. The second one is training the old classes using LMRC with Rehearsal extension. It is why we extend LMRC with Rehearsal in Sec.\ref{}.  Thus, we can conclude that this mixing setup is much easier than ours and it can be regarded as a special case of the setup in our paper. 
\subsection{The Universality of the Model}
LMRC can be regarded as a universal class incremental learning method, which can be adopted in many related fields.
In fact, LMRC only modifies the learning targets and the head part of the neural network.
The neural network structure is independent to LMRC.
\subsection{Estimation of P(A)}
In Sec.\ref{}, we assuem that

